Interactively Teaching an Inverse Reinforcement Learner with Limited Feedback

We study the problem of teaching via demonstrations in sequential decision-making tasks. In particular, we focus on the situation when the teacher has no access to the learner's model and policy, and the feedback from the learner is limited to trajectories that start from states selected by the teacher. The necessity to select the starting states and infer the learner's policy creates an opportunity for using the methods of inverse reinforcement learning and active learning by the teacher. In this work, we formalize the teaching process with limited feedback and propose an algorithm that solves this teaching problem. The algorithm uses a modified version of the active value-at-risk method to select the starting states, a modified maximum causal entropy algorithm to infer the policy, and the difficulty score ratio method to choose the teaching demonstrations. We test the algorithm in a synthetic car driving environment and conclude that the proposed algorithm is an effective solution when the learner's feedback is limited.

==> 4-teaching.tex <==

\section{Teaching with limited feedback} \label{chap:teaching}

In this section, we present our second contribution, the algorithm for teaching with limited feedback.
We first describe how the \ac{MCE-IRL} and Active-VaR algorithms can be modified to be compatible with the interactive teaching process.
We call these modified versions Interactive-MCE and Interactive-VaR, respectively.
Then we propose a teaching algorithm that combines Interactive-VaR, Interactive-MCE, and DSR into a compound algorithm which we call \acfi{TLimF}.

\input{4c-imce}

\input{4d-ivar}

\input{4e-tlimf}


==> paper.tex <==
\input{paper-ecai}
\typeout{get arXiv to do 4 passes: Label(s) may have changed. Rerun}

